A Unified Approach to Memory-Sample Tradeoffs for Detecting Planted Structures

We present a unified framework for proving memory lower bounds for multi-pass streaming algorithms that detect planted structures. Planted structures -- such as cliques or bicliques in graphs, and sparse signals in high-dimensional data -- arise in numerous applications, and our framework yields multi-pass memory lower bounds for many such fundamental settings. We show memory lower bounds for the planted $k$-biclique detection problem in random bipartite graphs and for detecting sparse Gaussian means. We also show the first memory-sample tradeoffs for the sparse principal component analysis (PCA) problem in the spiked covariance model. For all these problems to which we apply our unified framework, we obtain bounds which are nearly tight in the low, $O(\log n)$ memory regime. We also leverage our bounds to establish new multi-pass streaming lower bounds, in the vertex arrival model, for two well-studied graph streaming problems: approximating the size of the largest biclique and approximating the maximum density of bounded-size subgraphs. To show these bounds, we study a general distinguishing problem over matrices, where the goal is to distinguish a null distribution from one that plants an outlier distribution over a random submatrix. Our analysis builds on a new distributed data processing inequality that provides sufficient conditions for memory hardness in terms of the likelihood ratio between the averaged planted and null distributions. This result generalizes the inequality of [Braverman et al., STOC 2016] and may be of independent interest. The inequality enables us to measure information cost under the null distribution -- a key step for applying subsequent direct-sum-type arguments and incorporating the multi-pass information cost framework of [Braverman et al., STOC 2024].

==> gaussian_approx.tex <==
\section{Gaussian approximation to binomial}



\begin{theorem}
Let $P$ be the Binomial distribution on $n$ trials with bias $1/2$. Let $Q$ denote the discretized Gaussian distribution $N(n/2,n/4)$, with probability mass function given by,

\begin{align*}
    Q(i) = \int_{i-1/2}^{i+1/2} f_n(x) dx, \quad i \in \mathbb{I},\quad\text{with}\quad f_n(x)=\frac{2}{\sqrt{2\pi n}}\exp\Bigl\{-\frac{2(x-n/2)^2}{n}\Bigr\}.
\end{align*}
Then $D(P \parallel Q) \le C\log^2n/n$, for some constant $C>0$.

\end{theorem}

\begin{proof}

Let $P(i)$ denote the probability mass function of the binomial distribution $P$,
\begin{align*}
    P(i) = \binom{n}{i} 2^{-n},\quad i=0,1,\dots,n.
\end{align*}
Define the normalized and centered variable
\[
z=\frac{2(i-n/2)}{\sqrt{n}}.
\]
Our first step is to approximate the density of $P$ using the Gaussian. Local limit theorems such as the De Moivre–Laplace theorem (a special case of the central limit theorem) show that the density of $P$ asumpotically converges to the appropriate Gaussian. Here, we use a refined version of the local limit theorem which provides a bound on the rate of convergence. By Theorem 13 in \cite{petrov1975some} (also see the Wikipedia page on Edgeworth series), for any $k\ge 1$,
\begin{align}
P(i)=\frac{2}{\sqrt{2\pi n}}\exp\Bigl(-\frac{z^2}{2}\Bigr)\left[\sum_{\nu = 1}^{k}\frac{w_{\nu}(z)}{n^{\nu/2}} + o\left(\frac{1}{n^{k/2}}\right)  \right].\label{eq:edgeworth}
\end{align}
Here,
\[
w_{\nu}(z)=\sum H_{\nu + 2s} (z) \prod_{m=1}^{\nu} \frac{1}{k_m!}\left(\frac{\gamma_{m+2}}{(m+2)!\sigma^{m+2}}\right)^{k_m},
\]
where the summation on the right hand side is carried over all non-negative integer solutions $(k_1,\dots,k_{\nu})$ of the equalities $k_1+2k_2+\dots+\nu k_{\nu}=\nu$ and $s=k_1+\dots+k_{\nu}$, $\gamma_{i}$ denotes the $i$-th cumulant of the unbiased Bernoulli distribution $\text{Ber}(1/2)$, $\sigma=1/2$ is the standard deviation of $\text{Ber}(1/2)$, and  $H_{i}(z)$ is the $i$-th Chebyshev-Hermite polynomial.

We use \eqref{eq:edgeworth} with $k=2$. We first calculate $w_1(z)$, where the only term in the summation is $k_1=1$,
\begin{align*}
    w_1(z) = H_3(z)\cdot \frac{\gamma_3}{3!(1/2)^3}=0,
\end{align*}
where in the last step we use the fact that $\text{Ber}(1/2)$ is symmetric around its mean, and hence the third cumulant $\gamma_3=\bbE [ (X - \bbE[X])^3 ]$ for $X\sim \text{Ber}(1/2)$  is 0. The expansion for $w_2(z)$ involves $(k_1,k_2)\in\{(2,0),(0,1)\}$, and hence yields some polynomial $r(z)$ with constant coefficients and degree at most 4, since the highest order Chebyshev-Hermite polynomial which appears in the expansion is $H_4(z)$. Therefore on simplifying \eqref{eq:edgeworth} with $k=2$ we get the following expansion of the binomial pdf in terms of the Gaussian pdf,
\begin{align}
P(i)=\frac{2}{\sqrt{2\pi n}}\exp\Bigl(-\frac{z^2}{2}\Bigr)\left[1+\frac{r(z)}{n}+o\left(\frac{1}{n}\right)\right].\label{eq:binomial_approx}
\end{align}


Next, we approximate the discretized Gaussian density. We have
\[
Q(i)=\int_{i-1/2}^{i+1/2} f_n(x)\,dx,\qquad f_n(x)=\frac{2}{\sqrt{2\pi n}}\exp\Bigl\{-\frac{2(x-n/2)^2}{n}\Bigr\}.
\]
For $x=i+y$ with $y\in[-1/2,1/2]$, note that
\[
(x-n/2)^2=(i-n/2)^2+2y(i-n/2)+y^2.
\]
Thus,
\[
f_n(i+y)=\frac{2}{\sqrt{2\pi n}}\exp\Bigl\{-\frac{2(i-n/2)^2}{n}\Bigr\}\exp\Bigl\{-\frac{4y(i-n/2)+2y^2}{n}\Bigr\}.
\]
Define
\[
g(y)=-\frac{4y(i-n/2)+2y^2}{n}.
\]
A Taylor expansion of $\exp(g(y))$ yields
\[
\exp(g(y))=1+g(y)+R_g(y),
\]
where, 
\[
|R_g(y)|\le \frac{C_1}{n^{2}}\Bigl(1+|i-n/2|^2\Bigr),
\]
for some constant $C_1$, uniformly for $|y|\le 1/2$. Therefore for $|i-n/2|\le 5\sqrt{n\log n}$,
\begin{align*}
\int_{-1/2}^{1/2} \exp(g(y))\,dy &= \int_{-1/2}^{1/2} \,dy+\int_{-1/2}^{1/2}g(y)\,dy+\int_{-1/2}^{1/2}R_g(y)\,dy\\
&\ge 1-\frac{1}{6n}-\frac{C_1}{n^{2}}\Bigl(1+|i-n/2|^2\Bigr)\\
&\ge 1-\frac{C_2\log n}{n},
\end{align*}
for some constant $C_2$. Hence, for $|z|\le 10\sqrt{\log n}$,
\begin{align}
Q(i)\ge \frac{2}{\sqrt{2\pi n}}\exp\Bigl(-\frac{z^2}{2}\Bigr)\Bigl[1-\frac{C_2\log n}{n} \Bigr].\label{eq:discrete_gaussian}
\end{align}

We now analyze the ratio $\frac{P(i)}{Q(i)}$. Using \eqref{eq:binomial_approx} and \eqref{eq:discrete_gaussian}, for $|z|\le 10\sqrt{\log n}$ we can write,
\begin{align*}
\frac{P(i)}{Q(i)}&\le \frac{1+\frac{r(z)}{n}+o\left(\frac{1}{n}\right)}{1-\frac{C_2\log n}{n} }\\
&\le \left(1+\frac{r(z)}{n}+o\left(\frac{1}{n}\right)\right)\left(1+\frac{2C_2\log n}{n} \right) \quad \text{(since } 1/(1-x)\le 1+2x \text{ for } x \le 1/2)\\
&= 1+\frac{r(z)}{n}+\frac{2C_2\log n}{n}+\frac{2C_2r(z)\log n}{n^2}+o\left(\frac{1}{n}\right)\\
&\le 1+\frac{C_3\log^2 n}{n},
\end{align*}
where in the last step we use the fact $r(z)\le C'\log^2 n$ for some constant $C'$, since $r(z)$ has constant coefficients and degree at most 4, and $|z|\le 10\sqrt{\log n}$. Since $\log (1+x)\le 2x$ for sufficiently small $x$, we can write,
\begin{align*}
\log \left(\frac{P(i)}{Q(i)}\right)&\le \frac{2C_3\log^2 n}{n}.
\end{align*}

We now calculate the KL divergence contribution from the central region of the distribution, where most of the mass lies. Define the central region
\[
\mathcal{C}=\{i: |z|\le 10\sqrt{\log n}\}.
\]
Then
\begin{align}
\sum_{i\in\mathcal{C}}P(i)\log\frac{P(i)}{Q(i)}\le \sum_{i\in\mathcal{C}}P(i) \frac{2C_3\log^2 n}{n}\le \frac{2C_3\log^2 n}{n}.\label{eq:kl1}
\end{align}


Finally, we calculate the contribution from the tail. We first note that by a standard Chernoff bound, 
\begin{align}
\sum_{i\notin\mathcal{C}}P(i)\le 1/n^2.\label{eq:chernoff}
\end{align}

Next, note that $Q(i) \ge Q(0)$ for $0\le i \le n$. Moreover, 
\begin{align*}
    Q(0) \ge f_n(-1/2)= \frac{2}{\sqrt{2\pi n}}\exp\Bigl\{-\frac{2(-1/2-n/2)^2}{n}\Bigr\}\ge \exp(-10n),
\end{align*}
for $n$ sufficiently large. Therefore,
\begin{align}
\sum_{i\notin\mathcal{C}}P(i)\log\frac{P(i)}{Q(i)}\le \sum_{i\notin\mathcal{C}}P(i)\log\frac{1}{Q(i)}\le \sum_{i\notin\mathcal{C}}P(i)\cdot 10n\le 10/n,\label{eq:kl2}
\end{align}
where the last step uses \eqref{eq:chernoff}. Combining \eqref{eq:kl1} and  \eqref{eq:kl2} shows that 
\begin{align*}
    \sum_{0\le i \le n}P(i)\log\frac{P(i)}{Q(i)}\le \frac{C\log^2 n}{n}
\end{align*}
for some constant $C$, proving the theorem.

\end{proof}

==> tail_bounds.tex <==

\begin{proposition}[Tail Bound for Gaussian, \cite{Vershynin_2018}]
    Let $g \sim N(0, 1)$. Then for all $t < 0$, we have 
    \[
    \Pr \{ g \geq t \} \leq \frac{1}{t} \frac{1}{\sqrt{2 \pi}}  \exp ( - t^2 / 2 )
    \]
\end{proposition}
